Color Sails: Discrete-Continuous Palettes for Deep Color Exploration

We present color sails, a discrete-continuous color gamut representation that extends the color gradient analogy to three dimensions and allows interactive control of the color blending behavior. Our representation models a wide variety of color distributions in a compact manner, and lends itself to applications such as color exploration for graphic design, illustration and similar fields. We propose a Neural Network that can fit a color sail to any image. Then, the user can adjust color sail parameters to change the base colors, their blending behavior and the number of colors, exploring a wide range of options for the original design. In addition, we propose a Deep Learning model that learns to automatically segment an image into color-compatible alpha masks, each equipped with its own color sail. This allows targeted color exploration by either editing their corresponding color sails or using standard software packages. Our model is trained on a custom diverse dataset of art and design. We provide both quantitative evaluations, and a user study, demonstrating the effectiveness of color sail interaction. Interactive demos are available at www.colorsails.com.

==> analy.tex <==
Many 2D graphics created by artists and designers today are comprised of large numbers of colors, not well-represented by discrete color palettes. In order to design a flexible color gamut representation suitable for a variety of creative tasks, it is necessary to understand what kind of color gamuts naturally occur in 2D graphics. For example, a purely continuous representation, such as the one proposed in~\cite{shugrina2017playful}, may be a poor representation for domains, where discrete color choices are more meaningful. In order to gain a better understanding of the color gamuts that occur naturally in a variety of 2D graphics, we collect images of different styles and analyze their color distributions.   

\subsection{Image Datasets}

We are interested in supporting color work for creation of a wide range of 2D graphics, including painting, illustration, graphic design and visualization. The image datasets we collected span all of these categories, and are meant to show the range of color usage, not form a comprehensive collection of all possible 2D styles. We broadly categorize images into the following categories: 1) art, which includes painting and illustration, 2) graphic design, which includes more targeted use cases, such as poster and logo design, and user interface design, 3) visualization, where primary goal is to graphically show information. We include photography for reference, but are not targeting this visual style in our work, as editing natural images calls for a different set of tools.

To our knowledge, no existing dataset covers such a broad set of categories. Therefore, we have collected images from searches in various web sources, selecting a source based on how well the search results matched our target category in order to minimize manual clean up. For physical painting, we have used Google Search API~\cite{googlesearch} to collect 100 images by each of 30 well-known artists. For digital painting, we have used search query "digital painting" with a category "Painting" on \url{behance.net} \cite{behance}. For "illustration", we have collected images from the curated "Illustration" gallery on behance.net, and also collected images of New Yorker cover art~\cite{newyorker}, which spans a wide range of illustration styles. For poster graphic design, we searched pinterest.com~\cite{pinterest} for "poster design". For logo design, we searched designinspiration.com \cite{designinsp} for "logo design", and also collected logos of the Fortune 500 companies~\cite{fortune500}. For user interface design, we focused on mobile apps and searched pinterest.com for "app ux design" and collected screenshots from mobile-patterns.com \cite{mobilepatterns}. Because photographs are very common in UX mock ups and can skew color distributions, we have removed or masked most occurrences of photographs in UX design. For visualization, we have used an existing MassViz dataset of hand-labeled images~\cite{borkin2013makes}. Finally, for high-quality professional photography we have used images from the curated "Photography" gallery on behance.net. These datasets are summarized in Table~\ref{tb:data}.

\begin{table}[ht]
\begin{center}
\small{
\begin{tabular}{@{}c|l|l|c|c@{}}
\bf{Category} & \bf{Subcat.} & \bf{Src} & \bf{\#Orig.}  & \bf{\#Clean}  \\
\Xhline{1.3pt}
\multirow{3}{*}{\bf{Art}}&(A1) Phys.\ paint.&GS&2808&todo\\
\cline{2-5}
&(A2) Digital paint.&BH+DI&1075+1011&todo\\
\cline{2-5}
&(A3) Illustration&BH+NY&1046+2497&todo\\
\Xhline{0.8pt}
\multirow{3}{*}{\shortstack{\bf{Graphic} \\ \bf{Design}}}&(G1) Posters&PN&988&todo\\
\cline{2-5}
&(G2) Logos&DI+GS&1048+500&todo\\
\cline{2-5}
&(G3) UX design&PN+MP&933+1394&todo\\
\Xhline{0.8pt}
\bf{Viz.}&(V1) Misc.&MassViz&2000&2000\\
\Xhline{0.8pt}
\bf{Photo}&(P1) Misc.&BH&1078&todo\\
\Xhline{1.3pt}
\end{tabular}
}
\end{center}
\caption{\textbf{Image Datasets}: Data used for analysis, marked with original sources of the data, original number of images collected and number of images remaining after manual clean up. Source legend: BH - behance.net, DI - designspiration.net, GS - Google Search API, MP - mobile-patterns.com, MV - MassViz dataset~\cite{borkin2013makes}, NY - New Yorker covers from newyorker.com via Google Search API, PN - pinterest.com. }
\label{tb:data}
\end{table} 

\subsection{Analysis}

%We would like to understand, what kind of color gamut representations can cover this large variety of imagery. To this end, we make an observation that nearby pixel colors in a graphic are often related. 

As a first step, we analyze the number of colors used in different kinds of images. Simply counting unique RGB values in an image would yield meaningless results, as compression artifacts and interpolation during resizing can inflate the number of colors. To get a rough estimate, we perform agglomerative clustering of colors in LAB space until a maximum inter-cluster distance is reached (we use D=X, which is a barely perceptible difference to a human), and keep only the largest $N$ clusters accounting for 95\% of pixels in the image. $N$ is different for every image and we use it as a proxy for the true number of colors used to create the artwork.  

\begin{figure}[ht]
\centering
\subfloat[Infographic]{%
  \includegraphics[width=0.32\columnwidth]{fig/tmp_infogr.png}%
  }
\subfloat[Illustration]{%
  \includegraphics[width=0.32\columnwidth]{fig/octopus.png}%
  }
\subfloat[Painting]{%
  \includegraphics[width=0.32\columnwidth]{fig/tmp_medusa.jpeg}%
  }
\caption{Sample Images.}
\end{figure}


Merely plotting average number of colors used does not tell us how colors relate to each other. For example, large numbers of colors in a some UX designs could be due to a simple gradient, but the same number of colors in a digital painting is likely to include a more varied collection of hues. What we are after is figuring out what kind of low-dimensional color representations are well-suited to  

\subsection{Requirements for Color Gamut Representation}

Editable!

